A Novel Software-based Multi-path RDMA Solutionfor Data Center Networks

In this paper we propose Virtuoso, a purely software-based multi-path RDMA solution for data center networks (DCNs) to effectively utilize the rich multi-path topology for load balancing and reliability. As a "middleware" library operating at the user space, Virtuoso employs three innovative mechanisms to achieve its goal. In contrast to existing hardware-based MP-RDMA solution, Virtuoso can be readily deployed in DCNs with existing RDMA NICs. It also decouples path selection and load balancing mechanisms from hardware features, allowing DCN operators and applications to make flexible decisions by employing the best mechanisms (as "plug-in" software library modules) as needed. Our experiments show that Virtuoso is capable of fully utilizing multiple paths with negligible CPU overheads

==> implementation.tex <==
\section{Implementation}
We have implemented \mprdma{} as a user space ``middleware'' library on top of the standard RDMA libraries, \texttt{ib\_verbs} and \texttt{rdma\_cm}. \mprdma{} contains approximately 1500 lines of code (LoC) in C language.   \mprdma{} uses a thread-free method and event based mechanism  to handle multiple QPs establishment and data transmission.
An RDMA applications invokes \texttt{MP\_connect()} to create QP connections, and use \texttt{MP\_WRITE()/SEND()} to initiate a multipath data transmission. 
Additionally, we implemented two basic modules for congestion control and load balancing. However, they could be replaced easily for apps' own design.
